Unify and Anchor: A Context-Aware Transformer for Cross-Domain Time Series Forecasting

The rise of foundation models has revolutionized natural language processing and computer vision, yet their best practices to time series forecasting remains underexplored. Existing time series foundation models often adopt methodologies from these fields without addressing the unique characteristics of time series data. In this paper, we identify two key challenges in cross-domain time series forecasting: the complexity of temporal patterns and semantic misalignment. To tackle these issues, we propose the ``Unify and Anchor" transfer paradigm, which disentangles frequency components for a unified perspective and incorporates external context as domain anchors for guided adaptation. Based on this framework, we introduce ContexTST, a Transformer-based model that employs a time series coordinator for structured representation and the Transformer blocks with a context-informed mixture-of-experts mechanism for effective cross-domain generalization. Extensive experiments demonstrate that ContexTST advances state-of-the-art forecasting performance while achieving strong zero-shot transferability across diverse domains.

==> Tables/brif_few-shot_forecasting.tex <==
\begin{table*}[htbp]
\caption{The average forecasting results from 4 different prediction lengths \{96, 192, 336, 720\} in few-shot (5\% and 10\%) setting. The input length is set to 96. See Table for full results.}
\label{tab:brif_few_shot}
\vskip 0.05in
\centering
\resizebox{\textwidth}{!}{
\centering
\begin{threeparttable}
\renewcommand{\multirowsetup}{\centering}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{c|cc|cc|cc|cc|cc|cc||cc|cc|cc|cc|cc|cc}
\toprule
    Portion &  \multicolumn{12}{c||}{\rotatebox{0}{\scalebox{0.8}{\textbf{5\%}}}} & \multicolumn{12}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{10\%}}}}\\
\midrule
    \multirow{2}{*}{Models} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{ContexTST}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeXer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeMixer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{iTransformer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
    \multicolumn{2}{c||}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{ContexTST}}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeXer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeMixer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{iTransformer}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} \\

     & \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timexer}}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timemixer}}}&
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{liu2023itransformer}}}&
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{patchtst}}}&
    \multicolumn{2}{c||}{\scalebox{0.8}{\citeyear{wu2022timesnet}}} & \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timexer}}} &
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timemixer}}}&
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{liu2023itransformer}}}&
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{patchtst}}}&
    \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wu2022timesnet}}} \\

    \cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
    \cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}\cmidrule(lr){20-21}\cmidrule(lr){22-23}\cmidrule(lr){24-25}
    \scalebox{0.78}{Metric} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
\midrule
    \scalebox{0.85}{ETTh1} & \boldres{\scalebox{0.85}{0.705}}&\boldres{\scalebox{0.85}{0.572}}&\scalebox{0.85}{0.932}&\scalebox{0.85}{0.655}&\scalebox{0.85}{1.430}&\scalebox{0.85}{0.817}&\secondres{\scalebox{0.85}{0.914}}&\secondres{\scalebox{0.85}{0.649}}&\scalebox{0.85}{0.928}&\scalebox{0.85}{0.653}&\scalebox{0.85}{0.926}&\scalebox{0.85}{0.653} & \boldres{\scalebox{0.85}{0.698}}&\boldres{\scalebox{0.85}{0.558}}&\scalebox{0.85}{0.930}&\scalebox{0.85}{0.652}&\scalebox{0.85}{1.313}&\scalebox{0.85}{0.825}&\secondres{\scalebox{0.85}{0.908}}&\secondres{\scalebox{0.85}{0.640}}&\scalebox{0.85}{0.912}&\scalebox{0.85}{0.646}&\scalebox{0.85}{0.938}&\scalebox{0.85}{0.646}\\
    
    \scalebox{0.85}{ETTh2} &\boldres{\scalebox{0.85}{0.421}}&\boldres{\scalebox{0.85}{0.432}}&\scalebox{0.85}{0.484}&\scalebox{0.85}{0.467}&\scalebox{0.85}{0.661}&\scalebox{0.85}{0.546}&\secondres{\scalebox{0.85}{0.483}}&\secondres{\scalebox{0.85}{0.466}}&\scalebox{0.85}{0.484}&\scalebox{0.85}{0.471}&\scalebox{0.85}{0.485}&\scalebox{0.85}{0.469} &\boldres{\scalebox{0.85}{0.411}}&\boldres{\scalebox{0.85}{0.422}}&\scalebox{0.85}{0.476}&\scalebox{0.85}{0.461}&\scalebox{0.85}{0.645}&\scalebox{0.85}{0.517}&\secondres{\scalebox{0.85}{0.474}}&\scalebox{0.85}{0.463}&\scalebox{0.85}{0.477}&\scalebox{0.85}{0.464}&\scalebox{0.85}{0.480}&\secondres{\scalebox{0.85}{0.460}}\\

    \scalebox{0.85}{ETTm1} & \secondres{\scalebox{0.85}{0.718}}&\boldres{\scalebox{0.85}{0.563}}&\scalebox{0.85}{0.757}&\secondres{\scalebox{0.85}{0.572}}&\scalebox{0.85}{1.407}&\scalebox{0.85}{0.886}&\scalebox{0.85}{0.882}&\scalebox{0.85}{0.619}&\boldres{\scalebox{0.85}{0.692}}&\scalebox{0.85}{0.607}&\scalebox{0.85}{0.911}&\scalebox{0.85}{0.626} & \secondres{\scalebox{0.85}{0.312}}&\boldres{\scalebox{0.85}{0.332}}&\scalebox{0.85}{0.324}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.480}&\scalebox{0.85}{0.442}&\scalebox{0.85}{0.354}&\scalebox{0.85}{0.382}&\boldres{\scalebox{0.85}{0.307}}&\secondres{\scalebox{0.85}{0.345}}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.387}\\

    \scalebox{0.85}{ETTm2} & \boldres{\scalebox{0.85}{0.321}}&\secondres{\scalebox{0.85}{0.358}}&\scalebox{0.85}{0.339}&\scalebox{0.85}{0.371}&\scalebox{0.85}{0.507}&\scalebox{0.85}{0.465}&\scalebox{0.85}{0.355}&\scalebox{0.85}{0.383}&\secondres{\scalebox{0.85}{0.325}}&\boldres{\scalebox{0.85}{0.357}}&\scalebox{0.85}{0.362}&\scalebox{0.85}{0.388} & \secondres{\scalebox{0.85}{0.312}}&\boldres{\scalebox{0.85}{0.332}}&\scalebox{0.85}{0.324}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.480}&\scalebox{0.85}{0.442}&\scalebox{0.85}{0.354}&\scalebox{0.85}{0.382}&\boldres{\scalebox{0.85}{0.307}}&\secondres{\scalebox{0.85}{0.345}}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.387}\\

    \scalebox{0.85}{Electricity} & \boldres{\scalebox{0.85}{0.302}}&\boldres{\scalebox{0.85}{0.376}}&\scalebox{0.85}{0.325}&\scalebox{0.85}{0.400}&\scalebox{0.85}{0.324}&\scalebox{0.85}{0.390}&\scalebox{0.85}{0.316}&\scalebox{0.85}{0.391}&\secondres{\scalebox{0.85}{0.306}}&\secondres{\scalebox{0.85}{0.384}}&\scalebox{0.85}{0.372}&\scalebox{0.85}{0.457} & \boldres{\scalebox{0.85}{0.253}}&\boldres{\scalebox{0.85}{0.320}}&\scalebox{0.85}{0.298}&\scalebox{0.85}{0.375}&\scalebox{0.85}{0.282}&\scalebox{0.85}{0.366}&\scalebox{0.85}{0.276}&\scalebox{0.85}{0.358}&\secondres{\scalebox{0.85}{0.257}}&\secondres{\scalebox{0.85}{0.340}}&\scalebox{0.85}{0.362}&\scalebox{0.85}{0.448}\\

    \scalebox{0.85}{Weather} & \boldres{\scalebox{0.85}{0.291}}&\boldres{\scalebox{0.85}{0.317}}&\scalebox{0.85}{0.309}&\scalebox{0.85}{0.330}&\secondres{\scalebox{0.85}{0.300}}&\scalebox{0.85}{0.325}&\scalebox{0.85}{0.319}&\scalebox{0.85}{0.340}&\scalebox{0.85}{0.306}&\secondres{\scalebox{0.85}{0.324}}&\scalebox{0.85}{0.346}&\scalebox{0.85}{0.360} & \boldres{\scalebox{0.85}{0.287}}&\boldres{\scalebox{0.85}{0.312}}&\scalebox{0.85}{0.295}&\scalebox{0.85}{0.316}&\secondres{\scalebox{0.85}{0.292}}&\scalebox{0.85}{0.320}&\scalebox{0.85}{0.307}&\scalebox{0.85}{0.332}&\scalebox{0.85}{0.300}&\secondres{\scalebox{0.85}{0.315}}&\scalebox{0.85}{0.338}&\scalebox{0.85}{0.354}\\

    \scalebox{0.85}{Traffic} & \boldres{\scalebox{0.85}{0.813}}&\secondres{\scalebox{0.85}{0.539}}&\scalebox{0.85}{0.877}&\scalebox{0.85}{0.548}&\scalebox{0.85}{0.894}&\scalebox{0.85}{0.667}&\secondres{\scalebox{0.85}{0.872}}&\boldres{\scalebox{0.85}{0.536}}&\scalebox{0.85}{1.113}&\scalebox{0.85}{1.038}&\scalebox{0.85}{1.123}&\scalebox{0.85}{0.955} & \boldres{\scalebox{0.85}{0.754}}&\secondres{\scalebox{0.85}{0.489}}&\secondres{\scalebox{0.85}{0.777}}&\boldres{\scalebox{0.85}{0.483}}&\scalebox{0.85}{0.789}&\scalebox{0.85}{0.622}&\scalebox{0.85}{0.780}&\scalebox{0.85}{0.494}&\scalebox{0.85}{1.085}&\scalebox{0.85}{0.640}&\scalebox{0.85}{0.929}&\scalebox{0.85}{0.874}\\
\bottomrule
\end{tabular}
\end{threeparttable}
}
\end{table*}





% \begin{table*}[htbp]
% \caption{The average forecasting results from 4 different prediction lengths \{96, 192, 336, 720\} in few-shot (5\% and 10\%) setting. The input length is set to 96. See Table for full results.}
% \label{tab:brif_few_shot}
% \vskip 0.05in
% \centering
% \resizebox{\textwidth}{!}{
% \begin{subtable}
% \centering
% \begin{threeparttable}
% \renewcommand{\multirowsetup}{\centering}
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
% \toprule
%     \multirow{2}{*}{Models} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{ContexTST}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeXer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeMixer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{iTransformer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} \\

%      & \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timexer}}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timemixer}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{liu2023itransformer}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{patchtst}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wu2022timesnet}}} \\

%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
%     \scalebox{0.78}{Metric} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
% \midrule
%     \scalebox{0.85}{ETTh1} & \boldres{\scalebox{0.85}{0.705}}&\boldres{\scalebox{0.85}{0.572}}&\scalebox{0.85}{0.932}&\scalebox{0.85}{0.655}&\scalebox{0.85}{1.430}&\scalebox{0.85}{0.817}&\secondres{\scalebox{0.85}{0.914}}&\secondres{\scalebox{0.85}{0.649}}&\scalebox{0.85}{0.928}&\scalebox{0.85}{0.653}&\scalebox{0.85}{0.926}&\scalebox{0.85}{0.653}\\
    
%     \scalebox{0.85}{ETTh2} &\boldres{\scalebox{0.85}{0.421}}&\boldres{\scalebox{0.85}{0.432}}&\scalebox{0.85}{0.484}&\scalebox{0.85}{0.467}&\scalebox{0.85}{0.661}&\scalebox{0.85}{0.546}&\secondres{\scalebox{0.85}{0.483}}&\secondres{\scalebox{0.85}{0.466}}&\scalebox{0.85}{0.484}&\scalebox{0.85}{0.471}&\scalebox{0.85}{0.485}&\scalebox{0.85}{0.469}\\

%     \scalebox{0.85}{ETTm1} & \secondres{\scalebox{0.85}{0.718}}&\boldres{\scalebox{0.85}{0.563}}&\scalebox{0.85}{0.757}&\secondres{\scalebox{0.85}{0.572}}&\scalebox{0.85}{1.407}&\scalebox{0.85}{0.886}&\scalebox{0.85}{0.882}&\scalebox{0.85}{0.619}&\boldres{\scalebox{0.85}{0.692}}&\scalebox{0.85}{0.607}&\scalebox{0.85}{0.911}&\scalebox{0.85}{0.626}\\

%     \scalebox{0.85}{ETTm1} & \boldres{\scalebox{0.85}{0.321}}&\secondres{\scalebox{0.85}{0.358}}&\scalebox{0.85}{0.339}&\scalebox{0.85}{0.371}&\scalebox{0.85}{0.507}&\scalebox{0.85}{0.465}&\scalebox{0.85}{0.355}&\scalebox{0.85}{0.383}&\secondres{\scalebox{0.85}{0.325}}&\boldres{\scalebox{0.85}{0.357}}&\scalebox{0.85}{0.362}&\scalebox{0.85}{0.388}\\

%     \scalebox{0.85}{Electricity} & \boldres{\scalebox{0.85}{0.302}}&\boldres{\scalebox{0.85}{0.376}}&\scalebox{0.85}{0.325}&\scalebox{0.85}{0.400}&\scalebox{0.85}{0.324}&\scalebox{0.85}{0.390}&\scalebox{0.85}{0.316}&\scalebox{0.85}{0.391}&\secondres{\scalebox{0.85}{0.306}}&\secondres{\scalebox{0.85}{0.384}}&\scalebox{0.85}{0.372}&\scalebox{0.85}{0.457}\\

%     \scalebox{0.85}{Weather} & \boldres{\scalebox{0.85}{0.291}}&\boldres{\scalebox{0.85}{0.317}}&\scalebox{0.85}{0.309}&\scalebox{0.85}{0.330}&\secondres{\scalebox{0.85}{0.300}}&\scalebox{0.85}{0.325}&\scalebox{0.85}{0.319}&\scalebox{0.85}{0.340}&\scalebox{0.85}{0.306}&\secondres{\scalebox{0.85}{0.324}}&\scalebox{0.85}{0.346}&\scalebox{0.85}{0.360}\\

%     \scalebox{0.85}{Traffic} & \boldres{\scalebox{0.85}{0.813}}&\secondres{\scalebox{0.85}{0.539}}&\scalebox{0.85}{0.877}&\scalebox{0.85}{0.548}&\scalebox{0.85}{0.894}&\scalebox{0.85}{0.667}&\secondres{\scalebox{0.85}{0.872}}&\boldres{\scalebox{0.85}{0.536}}&\scalebox{0.85}{1.113}&\scalebox{0.85}{1.038}&\scalebox{0.85}{1.123}&\scalebox{0.85}{0.955}\\
% \bottomrule
% \end{tabular}
% \caption*{(a) Label Rate = 5\%}
% \label{tab:5_percent}
% \end{threeparttable}
% \end{subtable}
% \hfill
% \begin{subtable}
% \centering
% \begin{threeparttable}
% \renewcommand{\multirowsetup}{\centering}
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
% \toprule

%     \multirow{2}{*}{Models} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{ContexTST}}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeXer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeMixer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{iTransformer}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
%     \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} \\

%      & \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timexer}}} &
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2024timemixer}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{liu2023itransformer}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{patchtst}}}&
%     \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wu2022timesnet}}} \\

%     \cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
%     \scalebox{0.78}{Metric} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
% \midrule
%     \scalebox{0.85}{ETTh1} & \boldres{\scalebox{0.85}{0.698}}&\boldres{\scalebox{0.85}{0.558}}&\scalebox{0.85}{0.930}&\scalebox{0.85}{0.652}&\scalebox{0.85}{1.313}&\scalebox{0.85}{0.825}&\secondres{\scalebox{0.85}{0.908}}&\secondres{\scalebox{0.85}{0.640}}&\scalebox{0.85}{0.912}&\scalebox{0.85}{0.646}&\scalebox{0.85}{0.938}&\scalebox{0.85}{0.646}\\
    
%     \scalebox{0.85}{ETTh2} &\boldres{\scalebox{0.85}{0.411}}&\boldres{\scalebox{0.85}{0.422}}&\scalebox{0.85}{0.476}&\scalebox{0.85}{0.461}&\scalebox{0.85}{0.645}&\scalebox{0.85}{0.517}&\secondres{\scalebox{0.85}{0.474}}&\scalebox{0.85}{0.463}&\scalebox{0.85}{0.477}&\scalebox{0.85}{0.464}&\scalebox{0.85}{0.480}&\secondres{\scalebox{0.85}{0.460}}\\

%     \scalebox{0.85}{ETTm1} & \secondres{\scalebox{0.85}{0.616}}&\boldres{\scalebox{0.85}{0.509}}&\scalebox{0.85}{0.621}&\secondres{\scalebox{0.85}{0.519}}&\scalebox{0.85}{1.297}&\scalebox{0.85}{0.820}&\scalebox{0.85}{0.839}&\scalebox{0.85}{0.601}&\boldres{\scalebox{0.85}{0.580}}&\scalebox{0.85}{0.549}&\scalebox{0.85}{0.895}&\scalebox{0.85}{0.620}\\

%     \scalebox{0.85}{ETTm1} & \secondres{\scalebox{0.85}{0.312}}&\boldres{\scalebox{0.85}{0.332}}&\scalebox{0.85}{0.324}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.480}&\scalebox{0.85}{0.442}&\scalebox{0.85}{0.354}&\scalebox{0.85}{0.382}&\boldres{\scalebox{0.85}{0.307}}&\secondres{\scalebox{0.85}{0.345}}&\scalebox{0.85}{0.360}&\scalebox{0.85}{0.387}\\

%     \scalebox{0.85}{Electricity} & \boldres{\scalebox{0.85}{0.253}}&\boldres{\scalebox{0.85}{0.320}}&\scalebox{0.85}{0.298}&\scalebox{0.85}{0.375}&\scalebox{0.85}{0.282}&\scalebox{0.85}{0.366}&\scalebox{0.85}{0.276}&\scalebox{0.85}{0.358}&\secondres{\scalebox{0.85}{0.257}}&\secondres{\scalebox{0.85}{0.340}}&\scalebox{0.85}{0.362}&\scalebox{0.85}{0.448}\\

%     \scalebox{0.85}{Weather} & \boldres{\scalebox{0.85}{0.287}}&\boldres{\scalebox{0.85}{0.312}}&\scalebox{0.85}{0.295}&\scalebox{0.85}{0.316}&\secondres{\scalebox{0.85}{0.292}}&\scalebox{0.85}{0.320}&\scalebox{0.85}{0.307}&\scalebox{0.85}{0.332}&\scalebox{0.85}{0.300}&\secondres{\scalebox{0.85}{0.315}}&\scalebox{0.85}{0.338}&\scalebox{0.85}{0.354}\\

%     \scalebox{0.85}{Traffic} & \boldres{\scalebox{0.85}{0.754}}&\secondres{\scalebox{0.85}{0.489}}&\secondres{\scalebox{0.85}{0.777}}&\boldres{\scalebox{0.85}{0.483}}&\scalebox{0.85}{0.789}&\scalebox{0.85}{0.622}&\scalebox{0.85}{0.780}&\scalebox{0.85}{0.494}&\scalebox{0.85}{1.085}&\scalebox{0.85}{0.640}&\scalebox{0.85}{0.929}&\scalebox{0.85}{0.874}\\
    
% \bottomrule
% \end{tabular}
% \label{tab:10_percent}
% \caption*{(b) Label Rate = 10\%}
% \end{threeparttable}
% \end{subtable}
% }
% \end{table*}

